RoGSplat: Learning Robust Generalizable Human Gaussian Splatting from Sparse Multi-View Images

This paper presents RoGSplat, a novel approach for synthesizing high-fidelity novel views of unseen human from sparse multi-view images, while requiring no cumbersome per-subject optimization. Unlike previous methods that typically struggle with sparse views with few overlappings and are less effective in reconstructing complex human geometry, the proposed method enables robust reconstruction in such challenging conditions. Our key idea is to lift SMPL vertices to dense and reliable 3D prior points representing accurate human body geometry, and then regress human Gaussian parameters based on the points. To account for possible misalignment between SMPL model and images, we propose to predict image-aligned 3D prior points by leveraging both pixel-level features and voxel-level features, from which we regress the coarse Gaussians. To enhance the ability to capture high-frequency details, we further render depth maps from the coarse 3D Gaussians to help regress fine-grained pixel-wise Gaussians. Experiments on several benchmark datasets demonstrate that our method outperforms state-of-the-art methods in novel view synthesis and cross-dataset generalization. Our code is available at https://github.com/iSEE-Laboratory/RoGSplat.

==> figs/err.tex <==
\begin{figure}[h]
    \centering
    \includegraphics[width=\linewidth]{figs/rebuttal/err.pdf}
    \caption{\textbf{Error map of misalignment between 3D points and input images.} }
    \label{fig:err}
\end{figure}

==> figs/real_data.tex <==
\begin{figure}[ht]  
  \centering    
  \captionsetup[subfigure]{labelformat=empty,labelsep=space}
    \begin{subfigure}[c]{0.242\linewidth}		\includegraphics[width=1\textwidth, trim=160 30 180 30, clip]{figs/exp/real_data/nhp.png}
    \caption{NHP}
    \end{subfigure}
    \begin{subfigure}[c]{0.242\linewidth}		\includegraphics[width=1\textwidth, trim=160 30 180 30, clip]{figs/exp/real_data/th.png}
    \caption{TransHuman}
    \end{subfigure}
    \begin{subfigure}[c]{0.242\linewidth}		\includegraphics[width=1\textwidth, trim=160 30 180 30, clip]{figs/exp/real_data/gps.jpg}
    \caption{GPS-Gaussian}
    \end{subfigure}
    \begin{subfigure}[c]{0.242\linewidth}		\includegraphics[width=1\textwidth, trim=160 30 180 30, clip]{figs/exp/real_data/ours.jpg}
    \caption{Ours}
    \end{subfigure}
    
 \caption{\textbf{Qualitative comparison of cross-domain generalization.} We show the results trained with THuman2.0 and evaluated on real-world data~\cite{zheng2024gpsgaussian}.}
\label{fig:real_data}
\end{figure}

==> figs/seq.tex <==
\begin{figure}[h]
    
    \centering
    \vspace{-3mm}
    \includegraphics[width=\linewidth]{figs/rebuttal/seq.pdf}\\
    % \caption{\textbf{Results on sequential dataset.} }
    \label{fig:seq}
    \vspace{-6mm}
\end{figure}

==> figs/video.tex <==
\begin{figure}[h]
    \centering
    \vspace{-7mm}
    \includegraphics[width=\linewidth]{figs/rebuttal/video.pdf}\\
    %\caption{\textbf{Several frames from the supplementary video.} }
    \label{fig:video}
    \vspace{-4mm}
\end{figure}

==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    # if the dependency isn't one of the files that this latexmk run will consider, process it
    # without this test, we would get an infinite loop!
    if (!($root_filename eq $_[0]))
    {   # PLEASE ENABLE ONLY ONE OF THE FOLLOWING
        # DEPENDING ON THE ENGINE YOU'RE USING
    
        # FOR PDFLATEX
        system( "latexmk -pdf \"$_[0]\"" );

        # FOR LATEX+DVIPDF
        # system( "latexmk \"$_[0]\"" );

        # FOR XELATEX
        # system( "latexmk -xelatex \"$_[0]\"" );
        
        # FOR LUALATEX
        # system( "latexmk -lualatex \"$_[0]\"" );
   }
}


==> tables/ablate_random_rot.tex <==

\begin{table}[]
\centering

\resizebox{\linewidth}{!}
{
\begin{tabular}{l l c c c}
\toprule[1pt]
\multirow{1}{*}{Method}& \multicolumn{1}{c}{PSNR$\uparrow$}& \multicolumn{1}{c}{SSIM $\uparrow$}& \multicolumn{1}{c}{ LPIPS $\downarrow$}\\ 
\midrule
NHP~\cite{kwon2021neural}&29.61 (13.5\%) &0.9646 (2.03\%)  &0.0452 (29.4\%) \\
GP-NeRF~\cite{chen2022gpnerf}&27.77 (14.5\%)  &0.9532 (1.86\%)  &0.0568 (26.9\%) \\
TransHuman~\cite{Pan_2023_ICCV}&29.43 (9.4\%)  &0.9641 (1.76\%)  &0.0345 (34.6\%) \\
GHG~\cite{kwon2024ghg}&24.98 (16.8\%)  &0.9418 (3.22\%)  &0.0522 (40.2\%) \\
Ours&30.13 (\textbf{4.7\%})  &0.9666 (\textbf{0.54\%})  &0.0359 (\textbf{6.9\%}) \\

\bottomrule[1pt]
\end{tabular}
}
\caption{\textbf{The robustness to the SMPL model.} We show the quantitative results on THuman2.0 using GT SMPL model, and present the decline ratio when utilizing the inaccurate SMPL model relative to the ground-truth version.}

\label{table:ablate_rot}
\end{table}

==> tables/rebuttal/metric.tex <==
\begin{table}[h]
\centering
\vspace{-3mm}
\resizebox{\linewidth}{!}
{
\begin{tabular}{l c c c c c}
\toprule[1pt]
\multirow{1}{*}{Metric}& \multicolumn{1}{c}{NHP}& \multicolumn{1}{c}{TransHuman}& \multicolumn{1}{c}{ GPS-Gaussian}& \multicolumn{1}{c}{ GHG}& \multicolumn{1}{c}{ Ours}\\ 
\midrule
SSIM$\uparrow$ & 0.7483&0.7952 &0.8095&0.7916&\textbf{0.8140}\\
LPIPS$\downarrow$&0.2491 & 0.2115&0.1854&0.2194&\textbf{0.1820}\\
\bottomrule[1pt]
\end{tabular}
}
%\caption{\textbf{Metrics computed from cropped images.}
\vspace{-4.5mm}
\label{table:metric}
\end{table}
